Collisional thermometry for Gaussian systems

We investigate a quantum thermometry scheme based collision model with Gaussian systems. A key open question of these schemes concerns the scaling of the Quantum Fisher Information (QFI) with the number of ancillae. In qubit-based implementations this question is difficult to assess, due to the exponentially growing size of the Hilbert space. Here we focus on Gaussian collision models, which allow for the scaling of the QFI to be evaluated for arbitrarily large sizes. This numerical flexibility enables us to explore the thermometric properties of the model for a wide range of configurations. Despite the infinite Markov order of the stochastic process of the model, we provide a simple phenomenological analysis for the behavior of the QFI, estimating the asymptotic Fisher information density and how the transient effects of correlations for an increasing number of ancillae depend on the physical parameters of the model.

==> draft_contents.tex <==
*** Introduction ***

*** Collisional Model ***

Description of the main idea of thermometry. Description of gaussian states. Idea of using steady states.

Description of the Master Equation for the System-Environment interaction, implementation for gaussian states. 

Description of the Unitary for the System-Ancilla interaction, implementation for gaussian states. 

Stability of the steady state. 

Quantum thermometry. QFI. QFI for Gaussian systems. Maximal QFI for full thermalization; proposal of using the correlations.

==> introduction_draft.tex <==
The development of quantum technology depends crucially on the precise control of quantum systems. The ability to extract information from these systems is necessary to perform tasks of quantum error correction in quantum computation [REF], [MORE EXAMPLES].  Quantum metrology is the area of physics that studies the use of quantum systems as information probes.

In a quantum metrology design, there exists a quantum system described by some parameter that we want to estimate. This parameter might be, for example, the temperature or the spin [REF]. The system of interest is coupled to ancillae that function as probes. After the interaction, a measurement is made on the set of ancillae that allow the experimenter to determine the parameter. The theory of metrology is interested in optimising this procedure and determining limits in the precision of this estimation, as well as relating these limits to physical resources available to the experimenter, such as the number of ancillae and the strength of the couplings. In quantum metrology, the interest also lies in studying quantum resources, such as entanglement. 

In thermometry, the parameter of interest is the temperature of a bath. This has applications in quantum thermodynamics, material sciences, and even biology. One simple example of a quantum thermometry design is is the one in which the ancillae are let to fully thermalize with the system. After this, one estimates the temperature of the bath by measuring the temperature of the ancillae. If $N$ ancillae are used, the estimation for the temperature has a standard  $\Delta T$ that is bounded bellow by the Cramer-Rao thermal bound

\begin{equation}\label{fullthermalizationbound}
    \frac{\Delta_T^2}{T^2} \geq \frac{k_B}{N C_A}
\end{equation}

\noindent where $C_A$ is the thermal capacity of each ancilla. One natural question is whether it is possible to surpass the bound given by Eq. \eqref{fullthermalizationbound}. In the work [REF], this question was answered in the positive. There, a collisional model was used to describe the interaction of the ancillae with the bath. We also use a collisional model here, as described in Sec. [REF], but using Gaussian bosonic systems instead of qubits. 
